Predictive Uncertainty Quantification for Bird's Eye View Segmentation: A Benchmark and Novel Loss Function

The fusion of raw sensor data to create a Bird's Eye View (BEV) representation is critical for autonomous vehicle planning and control. Despite the growing interest in using deep learning models for BEV semantic segmentation, anticipating segmentation errors and enhancing the explainability of these models remain underexplored. This paper introduces a comprehensive benchmark for predictive uncertainty quantification in BEV segmentation, evaluating multiple uncertainty quantification methods across three popular datasets with three representative network architectures. Our study focuses on the effectiveness of quantified uncertainty in detecting misclassified and out-of-distribution (OOD) pixels while also improving model calibration. Through empirical analysis, we uncover challenges in existing uncertainty quantification methods and demonstrate the potential of evidential deep learning techniques, which capture both aleatoric and epistemic uncertainty. To address these challenges, we propose a novel loss function, Uncertainty-Focal-Cross-Entropy (UFCE), specifically designed for highly imbalanced data, along with a simple uncertainty-scaling regularization term that improves both uncertainty quantification and model calibration for BEV segmentation.

==> Conclusion.tex <==


This paper presents a comprehensive evaluation of various uncertainty quantification methods for BEVSS. %
Our findings reveal that current methods do not achieve satisfactory results in uncertainty quantification, particularly in OOD detection, highlighting the need for advancements in this domain. Inspired by the robust calibration properties of Focal Loss, we introduce the UFCE loss, which significantly enhances both segmentation accuracy and calibration. To address the poor performance in OOD detection, we propose an uncertainty quantification framework incorporating UFCE loss, evidential regularization with pseudo-OOD exposure, and vacuity scaling. Extensive experiments validate the effectiveness of our approach in improving OOD detection capabilities.

\textbf{Limitations}: Our study faces two primary limitations. First, Proposition 2 only considers weight updates for the last linear layer, neglecting the influence of earlier layers, which are essential for a comprehensive understanding of the weight update dynamics. Second, there are no analytical forms for the thresholds \(\tau_1(\alpha_{c^*}, \gamma)\) and \(\tau_2(\alpha_{c^*}, \gamma)\) in Proposition 2, necessitating empirical estimation that may limit the generalizability of our findings. Future work will extend the analysis to include all network layers and aim to derive these thresholds analytically.




==> RelatedWork.tex <==
Existing BEVSS methods follow two main approaches: Lift splat shoot (LSS)~\cite{ng2020bev, philion2020lift, Huang2021BEVDetHM} and transformer-based. ~\cite{zhou2022cross, peng2022bevsegformer}. This paper uses two representative methods, LSS~\cite{philion2020lift} and Cross-View Transformer (CVT)~\cite{zhou2022cross}, as the backbones of our study. 

\textbf{LSS} 
leverages raw pixel inputs from multiple surrounding cameras and ``lifts'' each image individually into a frustum of features. Initially, it predicts a categorical distribution over a predefined set of possible depths. Subsequently, the frustum of features is generated by multiplying the features with their predicted depth probability. By utilizing known camera calibration matrices for each camera, a point cloud of features in the ego coordinate space can be obtained. LSS then ``splats'' all the frustums into a rasterized bird's-eye-view grid using a PointPillar \cite{Lang2018PointPillarsFE} model. These splatted features are then fed into a decoder module to predict BEVSS.
The concept of transforming from camera pixels to 3D point clouds and subsequently to BEV pixels has inspired several subsequent models, such as BEVDet~\cite{Huang2021BEVDetHM} and {FIERY}~\cite{hu2021fiery}.


\textbf{CVT} takes a distinct approach by leveraging transformer architecture and cross-attention mechanism.
CVT begins by extracting features from multiple surrounding camera images using a pre-trained EfficientNet-B4\cite{Tan2019EfficientNetRM} model. These extracted features serve as the attention values in the subsequent cross-attention step. 
To create the attention keys, the features are concatenated with the camera-aware positional embedding. This positional embedding is constructed using known camera pose and intrinsic information, enabling the model to account for the specific characteristics of each camera.
The positional encoding of the BEV space serves as the queries during the cross attention process. 


==> rebuttal.tex <==
\newpage

\section{Rebuttal Materials}
\subsection{Second round to 6WJb}


\subsection{Second round to Dvo9}
\textbf{Comment}:
Thanks for the provided experiment and clarification on the motivation of the OOD benchmarking regarding my question 1 and 2. While for the weakness:

1. The focal loss is a well-known technique for addressing data-imbalance in computer vision, which I assume as a common knowledge. Applying this to BEVSS and your benchmark seems to be trivial contribution as stated in your logic. Though I admit the combination of that loss into specific task setting (BEVSS) requires effort, that didn't provide new knowledge to the community, so I assume that is not a core contribution in this paper.

2. Thanks for the table to clarify the setting, and this is of great importance to the performance of different models, whichi should be highlighted to avoid any confusion.

Overall my previous idea of this paper haven't changed much, that it is more of a study paper. But with those clarification I think it is above the acceptance threshold and hope it could contribute to the community to encourage further insight into this problem. I will change my rating to 6.

\textbf{Response}
Thank you so much for your encouraging feedback. We will clarify the related points in our future revised version. We appreciate your acknowledgment of focal loss as a widely utilized technique for addressing data imbalance in computer vision tasks. Traditionally, focal loss is designed to operate with deterministic class probability vectors produced by softmax neural networks, where these vectors are directly compared with true class labels. However, adapting focal loss for evidential neural networks (ENNs) introduces a unique challenge: ENNs output a Dirichlet distribution over class probability vectors. This stochastic nature renders the original focal loss formulation unsuitable for direct optimization as a loss function.
 
To overcome this limitation, we propose the **Uncertainty Focal Cross-Entropy (UFCE)** loss, which is defined as the expectation of focal loss under the Dirichlet distribution predicted by ENNs. Our work is the first to introduce this novel adaptation of focal loss specifically for ENNs, derive its analytical form, and demonstrate its theoretical and empirical advantages over the standard Uncertainty Cross-Entropy (UCE) loss. We believe the UFCE loss, with its theoretical foundations and empirical validation, offers significant insights and value to the research community. We apologize if these points were not sufficiently emphasized in the original submission and will ensure greater clarity in the revised manuscript.
 
To illustrate the loss functions, consider the $i$-th pixel in the bird’s-eye view (BEV). Let $\mathbf{X}$ represent the input camera images, $\mathbf{p}$ denote the class probability vector, and $\mathbf{y}$ be the one-hot encoded true class label for the pixel. The ENN predicts a Dirichlet distribution $\text{Dir}(\boldsymbol{\alpha})$ over $\mathbf{p}$, such that $\mathbf{p} \sim \text{Dir}(\boldsymbol{\alpha})$. Below, we define and discuss the relationships between four loss functions: cross-entropy (CE), focal loss, UCE, and our proposed UFCE loss.
 
1. **Cross-Entropy Loss (CE):**
   $$
   \mathcal{L}^{\text{CE}}(\mathbf{p}, \mathbf{y})  
   = -\sum_{c=1}^C y_c \log p_c.
   $$
 
2. **Focal Loss:**
   $$
   \mathcal{L}^{\text{Focal}}(\mathbf{p}, \mathbf{y} )  
   = -\sum_{c=1}^C (1 - p_c)^{\gamma} y_c \log p_c,
   $$
   where $\gamma$ is a hyperparameter. The focal loss emphasizes harder-to-classify examples by modulating the loss contribution of well-classified samples.
 
Both CE and focal loss are designed for deterministic class probability vectors $\mathbf{p}$, typically produced by softmax neural networks.
 
3. **Uncertainty Cross-Entropy Loss (UCE):**
   In ENNs, the output is a Dirichlet distribution $\text{Dir}(\boldsymbol{\alpha})$ over $\mathbf{p}$. The UCE loss generalizes CE by taking its expectation under this distribution:
   $$
   \mathcal{L}^{\text{UCE}}(\boldsymbol{\alpha}, \mathbf{y}) 
   = E_{\mathbf{p} \sim \text{Dir}(\boldsymbol{\alpha})} \left[ -\sum_{c=1}^C y_c \log p_c \right]
   = \sum_{c=1}^C y_c \left( \psi(\alpha_0) - \psi(\alpha_c) \right),
   $$
   where $\psi(\cdot)$ is the digamma function, $\alpha_0 = \sum_{c=1}^C \alpha_c$, and $\alpha_c$ represents the Dirichlet parameter for class $c$. This loss encourages high evidential support for the true class $\alpha_{c^*}$ while reducing it for others.
 
However, UCE does not account for data imbalance, limiting its effectiveness in such scenarios.
 
4. **Uncertainty Focal Cross-Entropy Loss (UFCE):**
   To address data imbalance in ENNs, we introduce the UFCE loss, defined as the expectation of focal loss under the Dirichlet distribution:
   $$
   \mathcal{L}^{\text{UFCE}}(\boldsymbol{\alpha}, \mathbf{y})  
   = E_{\mathbf{p} \sim \text{Dir}(\boldsymbol{\alpha})} \left[ -\sum_{c=1}^C (1 - p_c)^{\gamma} y_c \log p_c \right]
   = \frac{B(\alpha_{0}, \gamma)}{B(\alpha_0 - \alpha_{c^*}, \gamma)} 
      \left[ \psi(\alpha_0 + \gamma) - \psi(\alpha_{c^*}) \right],
   $$
   where $B(\cdot)$ is the Beta function and $\gamma$ is a hyperparameter. Notably, UFCE reduces to UCE when $\gamma = 0$.
 
In summary, the UFCE loss integrates the benefits of UCE with the ability to handle data imbalance, marking a significant advancement in training ENNs effectively. We will incorporate these clarifications and detailed insights into the revised version for enhanced understanding.

